DiGRAF: Diffeomorphic Graph-Adaptive Activation Function

In this paper, we propose a novel activation function tailored specifically for graph data in Graph Neural Networks (GNNs). Motivated by the need for graph-adaptive and flexible activation functions, we introduce DiGRAF, leveraging Continuous Piecewise-Affine Based (CPAB) transformations, which we augment with an additional GNN to learn a graph-adaptive diffeomorphic activation function in an end-to-end manner. In addition to its graph-adaptivity and flexibility, DiGRAF also possesses properties that are widely recognized as desirable for activation functions, such as differentiability, boundness within the domain, and computational efficiency. We conduct an extensive set of experiments across diverse datasets and tasks, demonstrating a consistent and superior performance of DiGRAF compared to traditional and graph-specific activation functions, highlighting its effectiveness as an activation function for GNNs. Our code is available at https://github.com/ipsitmantri/DiGRAF.

==> sections/introduction_old.tex <==
%% Motivation: Success of GNNs 
% despite exploration on different design choices such as the layer design or the architectural type, most architectures default to the standard choice of activation functions, such as relu
Graph Neural Networks (GNNs) have important applications, from social networks and recommendation systems to bioinformatics and chemical analysis~\citep{wu2022graph, zhang2021graph, reiser2022graph} (\citet{zhou2020graph,wu2022graph} provides more examples). 
Recent work on GNNs have focused on the design space of several key architectural aspects, such as how to combine various known design choices of GNNs~\citep{you2020design}, how to design more expressive message and non-message passing layers~\citep{xu2019how, morris2019weisfeiler, maron2019provably,li2022expressive}, new pooling layers~\citep{ying2018hierarchical,lee2019self,murphy2019relational,bianchi2020spectral,wang2020haar}, or positional and structural encodings~\citep{dwivedi2020benchmarking,rampavsek2022recipe,lim2023sign,eliasof2023graph}. Despite exploration of these different design choices, most architectures default to the standard choice of activation functions~\citep{kipf2017semisupervised, chen2020simple, xu2019how, morris2019weisfeiler}, such as ReLU, among a few others.

% Motivation: Importance of activation functions
Activation functions play a crucial role in deep neural networks by introducing non-linearities and allowing them to capture complex behavior. Therefore, the choice of the activation function can significantly impact the downstream performance of neural networks, as also shown in \citet{nwankpa2018activation}. Popular examples of activation functions are the renowned Tanh (hyperbolic tangent) \citep{hochreiter1997long} and ReLU \citep{fukushima1969visual}, that found a wide range of applications in various fields~\citep{kunc2024three, dubey2022activation}. 
%
Recent studies advocate for the need of thoughtfully using activation functions, and suggest to \emph{learn} activation functions. In the context of general neural networks, some well-known examples of learnable activation functions are MaxOut \citep{pmlr-v28-goodfellow13}, as well as Parametric ReLU (PReLU) \citep{he2015delving}. 
More recently, \citet{maiti2024adact} proposes a new type of MLPs using diverse types of activation functions.
In terms of GNNs, while activation functions are utilized within GNNs, it is customary to use off-the-shelf activation functions such as ReLU, which were not primarily designed for graph data. In efforts to fill this void, recent studies suggested to design and learn \emph{graph-designated} activation functions. Some examples include \citet{iancu2020graph} that proposes a max-median activation filter, GReLU \citep{zhang2022graph}, that extends PReLU into a graph-adaptive mechanism, and TAFS~\citep{xu2023tafs}, that learns a task-aware activation using a bi-level optimization approach. %While \citet{xu2023tafs} focuses on task-specific performance, it does not account for the graph structure. \citet{iancu2020graph} considers only the local information, which are neighbors within a specified range, rather than incorporating the entire graph architecture. 

% might not be able to fully leverage the rich varied topologies information in graph data. 

%% What is missing: **graph adaptivity** and why it is important, GReLU: piecewise. GD: structure changes, size changes, graph structure can be various. Explain graph adaptivity

While the aforementioned methods seem to offer improved performance compared to standard activation functions, there is still a lack of comprehensive evaluation on various types of datasets and tasks. In our experiments we see that there is not a clear answer as to which activation function is consistently effective. Furthermore, the underlying activation blueprint of various methods can be limited. For instance, while \citet{iancu2020graph} takes into consideration local neighborhoods of nodes in the graph, it applies a pre-determined activation based on maximum and median filtering. Also, GReLU relies on similar ideas presented in PReLU, and proposes to learn the slopes and biases of ReLU-like segments. This approach yields a piecewise linear activation, which is limited in its expressiveness, as we show in \cref{fig:approximate:expressive}. Additionally, GReLU operates on an individual node and channel basis. Despite efforts to reduce parameter count, the model remains parameter-intensive on a per-channel basis, resulting in a substantial computational load. 

% \textcolor{red}{can also say something about the amount of parameters in GReLU - it is per channel and quite heavy}. 

 \begin{figure}[t]
    \centering
    %\vspace{-10pt}
    \includegraphics[width=0.8\columnwidth]{figures/DiGAF_Structure.pdf}
    \caption{Illustration of a layer in the network. Given node feature $\mathbf{H}^{(l-1)}$ and the adjacency matrix $\mathbf{A}$, we feed them to a $\textsc{GNN}_{\textsc{layer}}^{(l)}$ to extract updated node features. Then the updated feature $\bar{\mathbf{H}}^{(l)}$ is passed to the activation function layer \ourmethod. $\textsc{GNN}_{\textsc{act}}$ utilizes both $\bar{\mathbf{H}}^{(l)}$ and $\mathbf{A}$ to determine the activation function parameters $\vtheta^{(l)}$. The computation of $\vtheta^{(l)}$, introduces graph adaptivity and enhances the expressiveness of the activation function $T^{(l)}$. A comprehensive discussion on this process is presented in Section \ref{sec:methods}.}
    \label{fig:structure}
\end{figure}

% The existing limitations:
% 1. \citet{iancu2020graph}: local neighbors + pre-determined filter
% 2. GReLU - ReLU like piecewise-linear
% 3. GReLU - parameter intensive
% Solve: "global" graph adaptive + more expressive

To address these existing limitations of expressiveness and inconsistent empirical performance, we propose \ourmethod\ - a trainable Diffeomorphism-based Graph Activation Function.
Specifically, \ourmethod\ offers a novel and general activation function framework that adapts dynamically to the input graph while leveraging the expressive power of diffeomorphisms, which are invertible, continuously differentiable, and, when applied to learning tasks, can outperform gradient-based optimization.~\citep{freifeld2017transformations} While learning general diffeomorphisms can be challenging \citep{allassonniere2010construction, allassonniere2015bayesian, zhang2016bayesian}, we harness the  Continuous Piecewise-Affine Based Transformations (CPAB) framework \citep{freifeld2015highly, freifeld2017transformations}, which was originally designed mostly for applications in signal processing and computer vision by learning grid transformations to tackle input alignment challenges. 
%
%In our \ourmethod\~integrates a nonlinear transformation within the activation function layer, effectively introducing nonlinearity into the network.
%
On the contrary, in our \ourmethod, we propose to view node features as points sampled on a 1-dimensional grid. From this perspective, a learned diffeomorphism using CPAB, applied to node features, offers favorable properties: (i) it is fully differentiable, (ii) it is bounded, (iii) it offers a flexible and input adaptive nonlinear transformation of the features.
% 1) True, It is diffeomophism; 2) We use zero boundary so true: v at 0 and 1 is 0, so T(0) = 0 and T(1) = 0, CPAB is increasing at n = 1; 3) If we use theta GNN True
%
%We will demonstrate that our model guarantees the desirable properties not limited to graph adaptivity and continuous differentiable discussed above. 
Furthermore, \ourmethod\ is computationally efficient, with linear complexity and the capability for easy parallelization, enabling its execution in sub-linear time, and it is invertible -- a feature not offered by other popular activation functions like ReLU.  Lastly, \ourmethod\ is designed to maintain node permutation equivariance, as is desired in GNNs. %In addition, our \ourmethod\ ensures increasing monotonicity and guarantees that the absolute difference between the transformed outputs is proportionally constrained by the absolute distance of the inputs, within a constant factor.

%Graph adaptivity is crucial in GNNs. Compared to data in computer vision or NLP, the graph data are weakly structured; even within the same dataset, each graph can exhibit a distinct structure. The size and connectivity of graphs can vary widely, necessitating an approach that can dynamically adapt to these changes.
%The research most related to ours is GReLU of \citet{zhang2022graph}, in which we both utilize the input graph’s adjacency matrix and feature values to dynamically generate parameters for the activation function. Nonetheless, GReLU’s structure is inherently piecewise linear with a fixed number of slopes, which limited expressiveness of their model to capture complex patterns in the data. 
% Moreover, their experiments only tested models with at most 2 segments.

% Limited Expressiveness: Only a certain number of functions that can be expressed as piecewise linear when fixing the number of different slopes. With a fixed number of slopes, the activation function may not be able to capture complex patterns in the data. 
% Non-Differentiability at Junction Points: Networks with piecewise linear activations can have infinitely many spurious local minima
% Monotonicity and Identity Beahbior: Piecewise linear functions are not constrained to be monotonic.

%Therefore, in this paper, we are interested in addressing the question of how to design an expressive, efficient, and graph aware activation function for GNNs.

%% What we do
%% We introduce a method and describe the properties 
% What we tried to fill the gap by desgin a mehtod that is graph adaptive, we borrow CPAB framework in the Computer vision for different purpose, we will demonstrate that it guarantees the desirable properties (graph adaptivity, ...) discussed above



%% Experiments 
To verify the effectiveness of \ourmethod, we conduct numerous experiments on \textcolor{red}{number of datasets} on various tasks, from node classification, to graph classification and regression. We compare the performance of \ourmethod\ to three types of baselines: traditional activation functions, trainable activation functions, and graph activation functions. According to our results, \ourmethod\ offers consistent performance along various datasets, as well as improved downstream accuracy -- reflecting the theoretical understanding and reasoning behind the design of \ourmethod.


%% Contributions
\textbf{Main contributions.} The contributions of this work as are summarized as follows:
\begin{enumerate*}[label=(\arabic*), leftmargin=*]
    \item A learnable graph adaptive activation function based on expressive and efficient diffeomorphisms -- \ourmethod.
    % \item A theoretical analysis of the properties of \ourmethod, providing understanding on its behavior and design choices.
    \item An analysis of the properties of \ourmethod\ informing the design rationale. 
    \item A broad and comprehensive experimental evaluation of \ourmethod\ and other activation functions. Our results indicate consistent and improved performance offered by \ourmethod.
\end{enumerate*}

%The rest of the paper is organized as follows. In Section ~\ref{sec:relatedwork}, we discuss related work GNNs, activation functions, and learnable diffeomorphisms. We then present \ourmethod, in Section~\ref{sec:methods}, which is followed by an analysis of its properties in Section~\ref{sec:theoritical_analysis}. We conduct extensive experiments on node classification and graph classification and regression tasks in Section~\ref{sec:experiments}. Finally, we discuss our conclusions in Section~\ref{sec:conclusion}.














